RoarGraph: A Projected Bipartite Graph for Efficient Cross-Modal Approximate Nearest Neighbor Search

Approximate Nearest Neighbor Search (ANNS) is a fundamental and critical component in many applications, including recommendation systems and large language model-based applications. With the advancement of multimodal neural models, which transform data from different modalities into a shared high-dimensional space as feature vectors, cross-modal ANNS aims to use the data vector from one modality (e.g., texts) as the query to retrieve the most similar items from another (e.g., images or videos). However, there is an inherent distribution gap between embeddings from different modalities, and cross-modal queries become Out-of-Distribution (OOD) to the base data. Consequently, state-of-the-art ANNS approaches suffer poor performance for OOD workloads. In this paper, we quantitatively analyze the properties of the OOD workloads to gain an understanding of their ANNS efficiency. Unlike single-modal workloads, we reveal OOD queries spatially deviate from base data, and the k-nearest neighbors of an OOD query are distant from each other in the embedding space. The property breaks the assumptions of existing ANNS approaches and mismatches their design for efficient search. With insights from the OOD workloads, we propose pRojected bipartite Graph (RoarGraph), an efficient ANNS graph index built under the guidance of query distribution. Extensive experiments show that RoarGraph significantly outperforms state-of-the-art approaches on modern cross-modal datasets, achieving up to 3.56x faster search speed at a 90% recall rate for OOD queries.

==> algorithms/beam-search.tex <==
\begin{algorithm}[!tbhp]
\SetAlgoLined
\LinesNumbered
\SetNoFillComment
\KwIn{Graph $G$, query $q$, result size k, seed node $s$, length of search queue $L$, distance function $\delta(\cdot,\cdot)$}
\KwOut{Approximate nearest neighbors of q}
    
    $Result \gets \emptyset$
    
    \tcp*{Ascending order based on distance}
    Priority Queue $PQ(L)$

    $PQ \gets (ep, \delta(q,ep))$

    \While{$PQ$ has unvisited node}{
        $v \gets PQ.top()$ and mark $v$ as visited
        
        Add unvisited nodes in $N_{out}(v)$ to $PQ$

        % $visit(closest)$
    }
    
    % \For{$v \in N_u$}{
    %     $V' \gets V' \cup \{v\}$ \tcp*{Add v to the set of projected vertices}
    %     $E' \gets E' \cup \{(v,w)\}$ for all $w \in N_u$ \tcp*{Add edges between v and all neighbors of u in V}
    % }
    $Result \gets PQ[:k]$
\Return $Result$
\caption{BeamSearch}
\label{alg:beamsearch}
\end{algorithm}

==> figures/bipartite-graph.tex <==
\begin{figure}[!thbp]
    \centering
    \includegraphics[width=\linewidth]{figures/Bipartite-graph-rename-query.pdf}
    \caption{A bipartite graph comprising queries (green nodes) and base data (blue nodes).}
    \label{fig:bipartite-example}
\end{figure}

==> figures/different-query-sets.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/different-query-embedding-set.pdf}
\caption{Evaluation of different query embedding sets.}
% , verifying the robustness of \graphname to conventional ANNS
    \label{fig:insertion-eval}
    \vspace{-0.4cm}
\end{figure}

==> figures/insertion-and-diff-query-sets.tex <==
\begin{figure}
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/insertion-recall-10-laion.pdf}
    \caption{Evaluation of different insertion proportions.}
    \label{fig:insertion-performance}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/different-query-embedding-set.pdf}
    \caption{Evaluation of different query sets in building index.}
    \label{fig:different-query-sets}
\end{minipage}
\end{figure}



==> figures/key-insights.tex <==
\begin{figure}[!thbp]
    \centering
    \includegraphics[width=\linewidth]{figures/key-insights-no-query.pdf}
\caption{An illustration of performance degradation in the graph index, with $S_{i}$ denoting different spheres in high-dimensional space.  Assuming a search starts from $p$ in $S_1$. (a) Three nearest neighbors to an ID query clustered within $S_{4}$, allowing for efficient filtering of irrelevant nodes in the larger sphere at each greedy step and converge to $S_4$ along path $(p,x,y,z)$. (b) Search space cannot be reduced for the OOD query as nearest neighbors are distributed across $S_2$ and $S_3$. Greedy routing fails to converge in a single direction, requiring to traverse more nodes.}
% \vspace{-0.6cm}
    \label{fig:key-insights}
\end{figure}

==> figures/method-framework.tex <==
\begin{figure}[!thbp]
    \centering
    \includegraphics[width=\linewidth]{figures/framework-bold.pdf}
\caption{An overview of \graphname construction. Green nodes represent queries, and nodes A-G represent base data.}
 % (a) queries and base data form a bipartite graph, node G is isolated because of not close enough to the query node. (b) The bipartite graph is projected onto base nodes, G remains isolated and no routing path to node B. (c)
    \label{fig:mehod-framework-previous}
\end{figure}

==> figures/revision-sufficient-query.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/sufficient-queries.pdf}
\caption{Data Vectors for \graphname.}
% \vspace{-0.6cm}
    \label{fig:sufficient-queries}
\end{figure}

==> sections/response.tex <==


\noindent
Dear Editor and Reviewers:

\vspace{0.2cm}
\noindent
Thank you for the effort in reviewing our manuscript xxx, "xxx". 
A short summary of your revision.

\vspace{0.2cm}
\noindent
Yours sincerely,

%\vspace{0.2cm}
\noindent
Author A, Author B...



\section*{Response to the Editor} 
\begin{cmt*}{}{}
Editor Comments.
\end{cmt*}

\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your response. \cite{schuhmann2022laion}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 1
\newpage
\section{Response to reviewer 1} 

%%%%%%%%%%%%% Comment 1.1
\begin{cmt}{}{}

Comments 1.1

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 1.1

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 1.0
\begin{cmt*}{}{}        %% use * when do not need enumerate

Comments

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 1.2
\begin{cmt}{}{}

Comments 1.2

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 1.2

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 1.3
\begin{cmt}{}{}

Comments 1.3

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 1.3

\vspace{0.3cm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 2
\newpage
\section{Response to reviewer 2}

%%%%%%%%%%%%% Comment 2.1
\begin{cmt}{}{}

Comments 2.1

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 2.1

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.2
\begin{cmt}{}{}

Comments 2.2

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 2.2

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.3
\begin{cmt}{}{}

Comments 2.3

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 2.3

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 2.4
\begin{cmt}{}{}

Comments 2.4

\end{cmt}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

Your Response 2.4

\vspace{0.3cm}


